Controllable User Dialogue Act Augmentation for Dialogue State Tracking

Prior work has demonstrated that data augmentation is useful for improving dialogue state tracking. However, there are many types of user utterances, while the prior method only considered the simplest one for augmentation, raising the concern about poor generalization capability. In order to better cover diverse dialogue acts and control the generation quality, this paper proposes controllable user dialogue act augmentation (CUDA-DST) to augment user utterances with diverse behaviors. With the augmented data, different state trackers gain improvement and show better robustness, achieving the state-of-the-art performance on MultiWOZ 2.1

==> related_work.tex <==
\subsection{Dialogue State Tracking}
Recent advances in modeling DST can be broadly categorized into 3 types: span prediction, question answering, and generation-based models.
The question answering-based models define natural language questions for each slot to query the model for the corresponding values~\cite{zhou2019multi,gao-etal-2020-machine,li-etal-2021-zero}.
\citeauthor{wu-etal-2019-transferable} proposes TRADE, which is able to perform zero-shot transfer between multiple domains via slot-value embeddings and a state generator.
SimpleTOD~\cite{hosseini2020simple} combines all components of a task-oriented dialogue system with a pre-trained language model.
TripPy~\cite{heck-etal-2020-trippy} categorizes value prediction into 7 types, and designs different prediction strategies for each type.
In this work, we follow the categorizations defined by TripPy to perform generalized augmentation for DST.


\paragraph{Data Augmentation}
Researchers have applied data augmentation techniques to dialogue state tracking to improve models' performance.
Several prior work has explored augmentation methods for zero-shot transfer~\cite{yoo-etal-2020-variational,campagna-etal-2020-zero,kim-etal-2021-neuralwoz}, while our work focuses on in-domain data augmentation where ample supervision is available.

The closest related work is CoCo~\cite{li2020coco}, a framework that uses T5 to generate user utterances given augmented dialogue states.
The main differences between CoCo and our method are:
1) CoCo is designed for generating counterfactual evaluation data, while we use a similar approach for data augmentation, and
2) CoCo only handles span-based values, while we propose a generalized approach that could handle all types of values.

% The Dialogue State Tracking (DST) problem is aim to solve the problem that the machines cannot realize the goal of a dialogue. 
% When the problem be proposed, the researchers usually use the rule-based method to build the model, but this kind of method cannot be used in ASR and SLU domain.
% Therefore, the DST models can keep tracking many different possible results.
% Most of the main DST models can be classified into two parts, the generative models and the discriminative models.
% The generative models combine the input and the dialogue states to generate the result.
% And the discriminative models use the dialogue states to get the probability in different scenario, and get the most possible result.
% In the DST domain, there are many models and papers.
% \subsection{TripPy}
% TripPy use the triple copy method to get the information in the dialogues, which is the user inputs, system inform memory and the different slot values.
% TripPy use the there different and simple information to get the very high performance in the DST domain, which reach the 55\% accuracy on the MultiWOZ 2.1 dataset, which is a very complex dataset in DST domain.
% TripPy is based on BERT model, and use the triple copy mechanism, masking method the make the performance from 42.6\% up to 55\% compared with the model only use the span prediction method.
% \subsection{SimpleTOD}
% In this paper, the author firstly use the end-to-end model to deal with the DST problem.
% Not like the other DST models always use many different methods to deal with the different part in the DST problems, SimpleTOD use only a transformer model to handle it, but it still get a good performance on the DST problem. 
% There is another point, the SimpleTOD model can deal with the DST problem with many noise.
% For example, it can give their DST model multiple choices and in most of the condition, the system can still give a correct answer.
% \subsection{COCO}
% In NLP domain, there are many augmentation method to make the models have more accuracy, and COCO use some methods to augment the performance of many different DST models. 
% COCO use different belief state and turn label to generate different scenario which may be only a few on the original dataset.
% In their experiment, they discovered that if use their generated dataset to test on the original TripPy model, the model will only get a very low performance.
% However, if they use the augmented dataset to train TripPy, the model will give them a relatively high performance on the original MultiWOZ dataset.
% Same as TriPpy, the TRADE model and SimpleTOD model also have the same result.
% From COCO, we discovered that we can use some similar augmentation method to improve the models in DST domain.
